Fake or Compromised? Making Sense of Malicious Clients in Federated Learning

Federated learning (FL) is a distributed machine learning paradigm that enables training models on decentralized data. The field of FL security against poisoning attacks is plagued with confusion due to the proliferation of research that makes different assumptions about the capabilities of adversaries and the adversary models they operate under. Our work aims to clarify this confusion by presenting a comprehensive analysis of the various poisoning attacks and defensive aggregation rules (AGRs) proposed in the literature, and connecting them under a common framework. To connect existing adversary models, we present a hybrid adversary model, which lies in the middle of the spectrum of adversaries, where the adversary compromises a few clients, trains a generative (e.g., DDPM) model with their compromised samples, and generates new synthetic data to solve an optimization for a stronger (e.g., cheaper, more practical) attack against different robust aggregation rules. By presenting the spectrum of FL adversaries, we aim to provide practitioners and researchers with a clear understanding of the different types of threats they need to consider when designing FL systems, and identify areas where further research is needed.

==> Data_poisoning.tex <==
% \section{Data poisoning attack}


==> defense.tex <==
\section{Adaptive Defense}
To defend against our proposed hybrid attack, we propose an adaptive defense strategy in this section. The defense is premised on the utilization of data stolen from compromised clients, which forms the core of the hybrid attack. By enabling compromised clients to detect and report their status, such as through malware detection, they can alert the server. The server, in turn, uses their training data to filter out malicious updates based on these compromised images.

We conducted an empirical study tracking the loss values of malicious and benign updates across two datasets: a union of all stolen data and a benign dataset crafted by splitting the test dataset into validation and test subsets. Our aim was to mirror the size of the stolen dataset in the validation dataset. Notably, in a CIFAR10 experiment with 0.5\% of clients compromised, this equated to approximately 223 data samples. We observed that malicious updates typically exhibit higher loss values on the stolen dataset compared to the validation dataset, while benign updates yield higher loss values on the stolen dataset compared to the validation dataset with a smaller gap.

Consequently, we designed a defensive mechanism at the server level, incorporating these observations. This mechanism involves projecting all updates to maintain an L2 norm below a predefined threshold and calculating a weighted average of the updates. The Weights of the each update is calculated by loss value of that update on stolen dataset divided by sum of two loses. In this way we give more weight to the updates that have a smaller loss on the stolen data (i.e., benign updates). 

Testing our defense on CIFAR10 distributed over 1000 clients in a scenario with 5 compromised clients out of 1000, where the adversary can control 106 fake clients revealed a modest improvement in global model accuracy, approximately 1\%. This outcome suggests that the synthetic data generated by DDPM closely mimics the diversity of classes, enabling adversaries to submit updates nearly indistinguishable from benign ones, gradually degrading global accuracy and hindering optimal model performance. Future work will focus on refining this defense algorithm to more effectively counteract such sophisticated hybrid attacks.
